A Compensation Mechanism for EV Flexibility Services using Discrete Utility Functions

Compensation mechanisms are used to counterbalance the discomfort suffered by users due to quality service issues. Such mechanisms are currently used for different purposes in the electrical power and energy sector, e.g., power quality and reliability. This paper proposes a compensation mechanism using EV flexibility management of a set of charging sessions managed by a charging point operator (CPO). Users' preferences and bilateral agreements with the CPO are modelled via discrete utility functions for the energy not served. A mathematical proof of the proposed compensation mechanism is given and applied to a test scenario using historical data from an office building with a parking lot in the Netherlands. Synthetic data for 400 charging sessions was generated using multivariate elliptical copulas to capture the complex dependency structures in EV charging data. Numerical results validate the usefulness of the proposed compensation mechanism as an attractive measure both for the CPO and the users in case of energy not served.

==> Notation.tex <==
\vspace{-5pt}
\noindent \emph{Sets}
\begin{description}[itemsep=0.2ex, labelwidth=1.2cm, leftmargin=1.4cm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \item[$\Omega_{b}$] Set of nodes
\item[$\Omega_{f}$] Set of phases \{A, B, C\}
\item[$\Omega_{g}$] Set of nodes with distributed generation (DG) units
\item[$\Omega_{l}$] Set of distribution lines
\end{description}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \emph{Parameters}
\begin{description}[itemsep=0.2ex, labelwidth=1.2cm, leftmargin=1.4cm]
\item[\normalfont$\rm{c}$$_g^{\rm{DG}}$] Unitary generation cost at DG unit $g$ [\$/kW]
\item[\normalfont$\rm{c}^{\rm{ES}}$] Unitary generation cost at the substation [\$/kW]
\item[\normalfont$\overline{\rm{I}}_{kj}$] Maximum current magnitude at line $kj$ [A]
\item[$\rm{P}$$_{k,f}^{\rm{D}}$] Active power demand at node $k$, phase $f$ [kW]
\item[$\overline{\rm{P}}$$_{g}$] Maximum active power by generator at bus $g$ [kW]
\item[$\underline{\rm{P}}$$_{g}$] Minimum active power by generator at bus $g$ [kW]
\item[\normalfont$\rm{pf}$$_{g}$] Minimum power factor at DG unit $g$.
\item[\normalfont$\rm{Q}$$_{k,f}^{\rm{D}}$\rule{0pt}{2.3ex}] Reactive power demand at node $k$, phase $f$ [kVAr]
\itemsep=0.20ex\item[\normalfont$\rm{R}$$_{kj,f,f'}$] Resistance of line $kj$ between phases $f$ and $f'$ [$\Omega$]
\item[\normalfont$\overline{\rm{V}}$\rule{0pt}{2.3ex}] Maximum voltage magnitude [pu]
\item[\normalfont$\underline{\rm{V}}$] Minimum voltage magnitude [pu]
\item[$\rm{X}$$_{kj,f,f'}] Reactance of line $kj$ between phases $f$ and $f'$ [$\Omega$]
\item[$\Theta$] Defined angle range [$^\circ$]
\end{description}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \emph{Variables}
\begin{description}[itemsep=0.2ex, labelwidth=1.2cm, leftmargin=1.4cm]
\item[$i^{\rm{r}}_{kj,f}$  $i^{\rm{i}}_{kj,f}$] Real and imaginary parts of the current at line $kj$, phase $f$ [A]
\item[$i^{\rm{r\,D}}_{k,f}$  $i^{\rm{i\,D}}_{k,f}$] Real and imaginary parts of the load current at node $k$, phase $f$ [A]
\item[$i^{\rm{r\,DG}}_{g,f}$  $i^{\rm{i\,DG}}_{g,f}$] Real and imaginary parts of the current at DG unit $g$, phase $f$ [A]
\item[$i^{\rm{r\,ES}}_{k,f}$  $i^{\rm{i\,ES}}_{k,f}$] Real and imaginary parts of the current at the substation bus $k$, phase $f$ [A]
\item[$P^{\rm{ES}}$$]  Active power injection at the substation [kW]
\item[{$P^{\rm{DG}}_{g}$ $Q^{\rm{DG}}_{g}$}]  Active and reactive power generations at DG unit $g$ [kW, kvar]
\item[$v^{\rm{r}}_{k,f}$  $v^{\rm{i}}_{k,f}$] Real and imaginary parts of the voltage at node $k$, phase $f$ [V] 
\item[$\mu_g$] Unit status of DG unit at bus $g$ 
\end{description}


